Improving SAGA via a Probabilistic Interpolation with Gradient Descent

We develop and analyze a new algorithm for empirical risk minimization, which is the key paradigm for training supervised machine learning models. Our method---SAGD---is based on a probabilistic interpolation of SAGA and gradient descent (GD). In particular, in each iteration we take a gradient step with probability $q$ and a SAGA step with probability $1-q$. We show that, surprisingly, the total expected complexity of the method (which is obtained by multiplying the number of iterations by the expected number of gradients computed in each iteration) is minimized for a non-trivial probability $q$. For example, for a well conditioned problem the choice $q=1/(n-1)^2$, where $n$ is the number of data samples, gives a method with an overall complexity which is better than both the complexity of GD and SAGA. We further generalize the results to a probabilistic interpolation of SAGA and minibatch SAGA, which allows us to compute both the optimal probability and the optimal minibatch size. While the theoretical improvement may not be large, the practical improvement is robustly present across all synthetic and real data we tested for, and can be substantial. Our theoretical results suggest that for this optimal minibatch size our method achieves linear speedup in minibatch size, which is of key practical importance as minibatch implementations are used to train machine learning models in practice. Moreover, empirical evidence suggest that a linear speedup in minibatch size can be attained with a parallel implementation.

==> sections/overview_jacsketch.tex <==
\section{A Brief Overview of JackSketch}



The recently proposed JackSketch was motivated by several advances in randomized numerical linear algebra. The algorithm is based on two steps. The first is estimating the full jacobian of [] through sketch and project approaches while the second is to estimate the gradient. Note that the gradient of $f(\mathbf{x})$ can be computed through the jacobian as $\frac{1}{n} \nabla \mathbf{F}(\mathbf{x})\mathbf{e} = \nabla f(\mathbf{x})$ where $\nabla \mathbf{F}(\mathbf{x}) \stackrel{def}{=} \begin{bmatrix}\nabla f_1(\mathbf{x}), \dots, \nabla f_n(\mathbf{x}) \end{bmatrix}$ and $\mathbf{e}$ is the vector of all ones. JacSketch estimates the jacobian $\nabla \mathbf{F}(\mathbf{x})$ through means of sketch and project where for some positive definite weight matrix $\mathbf{W} \in \mathbb{R}^{n \times n}$:

\peter{Use $\mJ$ instead of $\mathbf{J}$. Do this for every matrix.}

\begin{equation}
    \begin{aligned}
    \mathbf{J}^{k+1} = \argmin_{\mathbf{J}^{d \times n}} \|\mathbf{J} - \mathbf{J}^k \|^2_{\mathbf{W}^{-1}} \\
    \text{s.t.} ~~ \mathbf{J} \mathbf{S}_k = \nabla \mathbf{F}(\mathbf{x}^k) \mathbf{S}_k
    \end{aligned}
\end{equation}

where $\|\mathbf{X}\|^2_{\mathbf{W}^{-1}} = \mathbf{X}\mathbf{W}^{-1} \mathbf{X}^\top$. 

\peter{Be careful how you define the norm. These kinds of typos should not really happen. Read what you write. We do not need $\mW$ as we only use $\mW=\mI$.}

The previous problem exhibits a closed form solution of the form:

\begin{equation}
    \begin{aligned}
    \mathbf{J}^{k+1} = \mathbf{J}^k + \left(\nabla \mathbf{F}(\mathbf{x}^k) - \mathbf{J}^k\right) {\bf \Pi}_{\mathbf{S}_k}
    \end{aligned}
\end{equation}
where
\begin{equation}
    \begin{aligned}
    {\bf\Pi}_{\mathbf{S}} \eqdef \mathbf{S}\left(\mathbf{S}^\top \mathbf{W} \mathbf{S}\right)^\dagger \mathbf{S}^\top \mathbf{W}
    \end{aligned}
\end{equation}

\peter{Use the $\eqdef$ macro  instead of $\stackrel{def}{=}$.}

This step of Jacobian estimate is later followed by a gradient estimate. To have an unbiased estimator of the gradient, they have introducted the stochastic relaxation parameters $\theta_{\mathbf{S}_k}$ satisfying $\mathbb{E}\left[\theta_{\mathbf{S}_k} {\bf \Pi}_{\mathbf{S}_k} \mathbf{e}\right] = \mathbf{e}$. Afterwards, they perform a standard gradient descent step with constant step sizes $\mathbf{x}^{k+1} \leftarrow \mathbf{x}^k - \alpha \mathbf{g}^k$ where the gradient estimate is given as follows:

\begin{equation}
    \begin{aligned}
    \mathbf{g^k} \eqdef \frac{1}{n} \mathbf{J}^k \mathbf{e} + \frac{1}{n} \left(\nabla \mathbf{F}(\mathbf{x}^k) - \mathbf{J}^k\right) \theta_{\mathbf{S}_k} \Pi_{\mathbf{S}_k} \mathbf{e}
    \end{aligned}
\end{equation}

Under different choices of sampling strategies several other well known algorithms arise as special cases. The celebrated SAGA for instance is a special case of JackSketch for when $\mathbf{W} = \mathbf{I}_n$ $\mathbf{S}_k = \mathbf{e}_k$ where $\mathbf{e}_k$ is the vector of all zeros but for the $k^{\text{th}}$ coordinate with a value of one.  Moreover, if $\mathbf{W} = \mathbf{I}_n$ and $\mathbf{S} = \mathbf{I}_{\mathbf{S}_k}$ where $\mathbf{I}_{\mathbf{S}_k}$ is a random column submatrix of the $n \times n$ identity matrix with columns indexd by $\mathbf{S}_k$ that is a subset of $[n]$, minibatch SAGA arises as special case. Lastly, when $\mathbf{W} = \mathbf{I}_n$ and $\mathbf{S}_k = \mathbf{I}_n$, JackSketch reduces to standard gradient descent. It has been shown for that JacSketch has a linear rate where if $\alpha = \min \left\{\frac{1}{4 \cL_1}, \frac{\kappa}{4 \cL_2 \rho / n^2 + \mu} \right\}$ the iteration complexity is $k \ge \max \left\{\frac{1}{\kappa} + \frac{4\rho \cL_2}{\kappa \mu n^2}, \frac{4 \cL_1}{\mu}\right\} \text{log}\left(\frac{1}{\epsilon}\right)$ to achieve $\epsilon$ accuracy in the sense that $\mathbb{E}\left[\Psi^k\right] \leq \epsilon \Psi^0$ where $\Psi^k = \|\mathbf{x}^k - \mathbf{x}^* \|_2^2 + \frac{\alpha}{2 \cL_2}\|\mathbf{J}^k - \nabla \mathbf{F}(\mathbf{x}^*) \|_{\mathbf{W}^{-1}}$.


